Simpler Does It: Generating Semantic Labels with Objectness Guidance

Existing weakly or semi-supervised semantic segmentation methods utilize image or box-level supervision to generate pseudo-labels for weakly labeled images. However, due to the lack of strong supervision, the generated pseudo-labels are often noisy near the object boundaries, which severely impacts the network's ability to learn strong representations. To address this problem, we present a novel framework that generates pseudo-labels for training images, which are then used to train a segmentation model. To generate pseudo-labels, we combine information from: (i) a class agnostic objectness network that learns to recognize object-like regions, and (ii) either image-level or bounding box annotations. We show the efficacy of our approach by demonstrating how the objectness network can naturally be leveraged to generate object-like regions for unseen categories. We then propose an end-to-end multi-task learning strategy, that jointly learns to segment semantics and objectness using the generated pseudo-labels. Extensive experiments demonstrate the high quality of our generated pseudo-labels and effectiveness of the proposed framework in a variety of domains. Our approach achieves better or competitive performance compared to existing weakly-supervised and semi-supervised methods.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> related_work.tex <==
\vspace{-0.2cm}
\section{Related Work}\label{sec:related}
%Dense image labeling is an important task for many applications (e.g., autonomous vehicles, scene understanding, robotics, tumor segmentation). 
%In recent years, convolutional neural networks (CNNs)~\cite{krizhevsky12_nips,simonyan15_iclr,szegedy2015going,he2016deep} have proven to be the best candidate for semantic segmentation. 
%xisting works~\cite{krizhevsky12_nips,simonyan15_iclr,szegedy2015going,he2016deep,long15_cvpr,chen15_iclr,noh15_iccv,badrinarayanan15_arxiv,ghiasi2016laplacian,chen2017rethinking} have achieved a high degree of success on dense image prediction tasks on standard benchmarks.
Due to the strenuous, time consuming, and costly nature of obtaining pixel-wise annotations, it is difficult to apply fully-supervised semantic segmentation~\cite{krizhevsky12_nips,simonyan15_iclr,szegedy2015going,he2016deep,long15_cvpr,chen15_iclr,noh15_iccv,badrinarayanan15_arxiv,ghiasi2016laplacian,chen2017rethinking} in real-world scenarios. To address this problem, WSSS and SSSS techniques with varying levels of supervision have been explored and have achieved promising performance. 
%Among the different types of supervision available, methods mostly rely on image or bounding box level supervision. 

%They have strong abilities to learn low-level and high-level features that enable them the identify the various objects within an image. Many variants have been proposed [CITE] for both supervised scenarios where every pixel per image is annotated by human annotators as well as weakly supervised cases, where some form of higher level annotation is used. 

%Existing WSSS methods~\cite{dai2015boxsup,lin2016scribblesup,fan2018associating,pathak2015constrained,wei2016stc,oh2017exploiting,chaudhry2017discovering,ahn2018learning,wei2018revisiting,wang2018weakly,huang2018weakly,hou2018self,song2019box} have considered various forms of weak supervision, including image labels~\cite{papandreou2015weakly,pathak2015constrained,qi2016augmented,lee2019frame,lee2019ficklenet}, bounding boxes~\cite{dai2015boxsup,khoreva2017simple,song2019box}, scribbles~\cite{lin2016scribblesup}, points~\cite{bearman2016s}, and class agnostic saliency~\cite{oh2017exploiting,shimoda2016distinct,zeng2019joint,wei2018revisiting}). Others have considered semi-supervised settings where only part of the data is labeled~\cite{xu2015learning}. 

\begin{figure*} [t]
	\begin{center}
		\includegraphics[width=0.98\textwidth]{figures/network.pdf}
	    \vspace{-0.25cm}
		\caption{\textbf{Overview of our proposed pipeline} consisting of pseudo-label generation (A) and Semantic Objectness Network (SONet) (B). For the pseudo-label generation: we learn an objectness classifier ($\mathcal{\phi_P}$) using the source dataset ($\mathcal{D_S}$). We generate pseudo-labels based on either the CAM ($\mathcal{G}^{_{\mathcal{C}_m}}$) or bounding box annotations ($\mathcal{G}^{_{\mathcal{B}}}$), with the class agnostic objectness prior ($\mathcal{O}$) obtained from the learned model. We spatially mask (denoted as $\odot$) the CAM or bounding boxes with the objectness prior using Eq.~\ref{eq:cam} and Eq.~\ref{eq:box} respectively. (B) With the generated pseudo-labels, we jointly train SONet, $\phi_O(\phi_\mathcal{S})$, on the target dataset, $\mathcal{D_T}$, to predict semantics, $\mathcal{S}$, and objectness, $\mathcal{S_O}$.}
		\label{fig:network}
	\end{center}
	\vspace{-0.5cm}
\end{figure*}
\noindent \textbf{Weakly-Supervised  Approaches.}
The majority of weakly-supervised approaches attempt to learn the segmentation model using image-level class labels or box-level proposals as supervision due to the ease of data collection compared with other types of labelling, such as pixel-level annotations. The most successful algorithm used to obtain semantic region proposals from image-level labels is the Class Activation Map (CAM)~\cite{zhou2016learning}. A drawback of CAM is that it frequently fails to capture detailed object boundaries, e.g., extremities or bike wheels. To address this problem, recent methods have used extra guidance to acquire better shape information, such as motion cues from video~\cite{hong2017weakly,lee2019frame,tokmakov2016learning}, class agnostic boundary proposals~\cite{ahn2018learning,qi2016augmented,papandreou2015weakly} and class agnostic saliency prior~\cite{fan2018associating,huang2018weakly,zeng2019joint,oh2017exploiting,zeng2019joint,wei2018revisiting}. Another line of works use bounding box proposals as weak supervision because they are relatively easy to annotate and offer strong semantic priors. They have previously been used in many ways for the task of generating semantic segmentation pseudo-labels~\cite{song2019box,dai2015boxsup,khoreva2017simple}. Most of the methods generate object proposals by applying either a CRF~\cite{krahenbuhl2011efficient} or GrabCut~\cite{rother2004grabcut} techniques to the bounding box annotations. Some works~\cite{dai2015boxsup,khoreva2017simple} introduced iterative techniques using the segment proposals as weak supervision. These approaches often have issues obtaining robust boundaries for non-salient regions within each bounding box. 

%^For instance,~\cite{zeng2019joint} recently proposed a multi-stage joint learning-based method for segmenting objects using true saliency annotations. Iterative methods have also been used without the requirement of additional information; however, these approaches are computationally expensive since they require many iterations to acquire the pseudo-label of a single image.\\
\noindent  \textbf{Semi-Supervised Approaches.} Semi-supervised approaches~\cite{lee2019ficklenet,huang2018weakly, wei2018revisiting} have the same end goal as WSSS but exploit a limited number of strong annotations (i.e., semantic segmentation groundtruth) from the dataset during the training phase. To leverage the images without groundtruth semantic segmentation annotations, many SSSS approaches also utilize CAMs or boundary box proposals to generate additional pseudo-labels. One limitation of SSSS methods is that the performance will decay when the amount of labeled data is not large enough or when the generated pseudo-labels are too noisy.

% Bounding boxes are appealing to use as supervision because they are relatively easy to annotate and offer strong semantic priors. They have previously been used in many ways for the task of generating semantic segmentation pseudo-labels~\cite{song2019box,dai2015boxsup,khoreva2017simple}. Most of the methods generate object proposals by applying either a CRF~\cite{krahenbuhl2011efficient} or GrabCut~\cite{rother2004grabcut} techniques to the bounding box annotations. Some works~\cite{dai2015boxsup,khoreva2017simple} introduced iterative techniques using the segment proposals as weak supervision. For instance, BCM~\cite{song2019box} generated pseudo-labels by first applying a CRF to bounding box annotations and then a per-class `filling rate' guided loss to produce their final prediction. These approaches often have issues obtaining robust boundaries for non-salient regions within each bounding box. 


% CAMs project the weights from a single class of the output logits, backwards through the network and back onto the input image, approximating likely object regions by drawing attention to discriminative parts of object classes. 
% To address common issues of poor boundary detail and inefficient pseudo-label generation, we propose an \emph{objectness} driven approach to remove object-irrelevant regions from semantic proposals before learning to segment. Our novel pseudo-label generation technique and joint learning framework produces performance very close to that of the fully supervised setting, allowing future research to be built upon our method. 
Our work is closely related to the approaches that use saliency information as additional guidance \cite{oh2017exploiting,wei2018revisiting,zeng2019joint,yao2020saliency} to generate pseudolabels for WSSS or SSSS. 
We argue that the use of saliency models for pixel-level boundary information is problematic, since the centre bias~\cite{bruce2015computational, accik2014real} causes salient region proposals to always be located near the image centre, thus the objects at the boundary will be incorrectly labelled as background (see Sec.~\ref{sec:SONet_abl}). In contrast, our objectness model learns to generate masks for objects at all image locations.  In addition, unlike SSSS methods, our approach does not require pixel-level semantic annotations; however we compare our approach with SSSS methods since the dataset used to generate the class-agnostic objectness guidance may have overlapping objects with the target dataset. 

To address common issues of poor boundary detail and inefficient generation of pseudo-labels, our \emph{objectness} driven approach removes object-irrelevant regions from semantic proposals before learning to segment. A single forward pass followed by a masking step generates each image's pseudo-labels giving highly accurate boundaries and enables practitioners to easily generate semantic segmentation pseudo-labels for new datasets in a variety of domains. 
%Our learning module, dubbed `SONet', is trained end-to-end, and jointly learns to predict semantics and objectness, making full use of the pseudo-label generation process.
 
 %\blue{SSSS studies~\cite{lee2019ficklenet,huang2018weakly,long15_cvpr} requires a ``small'' amount of labelled data as a start point for training. The labelled data can be viewed as a subset of the total dataset, thus there is an overlap of semantic information between the training and test data. Wei \textit{et al.}~\cite{wei2018revisiting} applied different sizes of dilated convolutional filters to combine the CAM information for SSSS. Huang \textit{et al.}~\cite{huang2018weakly} utilized CAM to locate initial semantic regions and expand the region by seed growing. Lee \textit{et al.}~\cite{lee2019ficklenet} also applied CAM for initial seed region but they proposed to grow the region with a separate network. One limitation of SSSS methods is that the performance will decay when the labelled data is not large enough. In this paper, our method does not require the pixel-level semantic annotation. Similar to saliency-based WSSS methods, our system only uses the binary mask of the COCO-stuff dataset as a boundary guidance. We compare our method against those SSSS methods because the category of the guidance may overlap with test data. (This may happen to those saliency-based WSSS too.) However, our method applies a weaker supervision than the SSSS setting.}
 
 %		\caption{Overview of our proposed pipeline consisting of pseudo-label generation (a,b,c) and Semantic Objectnes Network (d). For pseudo-label generation: (a) we learn an objectness predictor ($\mathcal{\phi_P}$) using the proxy dataset ($\mathcal{P}$). (b, c) we generate pseudo-labels based on either the CAM ($\mathcal{G}^{_{\mathcal{C}_m}}$) or bounding box annotations ($\mathcal{G}^{_{\mathcal{B}}}$), with the objectness mask obtained from the learned model in (a). We spatially mask (denoted as $\odot$) the CAM or bounding boxes with the objectness mask to remove non-overlapping pixels from the semantic region proposals. (d) With the generated pseudo-labels, we jointly train a segmentation objectness network on the source dataset, $\mathcal{D}_s$, to predict semantics and objectness.}
